MR-Scout: Automated Synthesis of Metamorphic Relations from Existing Test Cases

Metamorphic Testing (MT) alleviates the oracle problem by defining oracles based on metamorphic relations (MRs), that govern multiple related inputs and their outputs. However, designing MRs is challenging, as it requires domain-specific knowledge. This hinders the widespread adoption of MT. We observe that developer-written test cases can embed domain knowledge that encodes MRs. Such encoded MRs could be synthesized for testing not only their original programs but also other programs that share similar functionalities. In this paper, we propose MR-Scout to automatically synthesize MRs from test cases in open-source software (OSS) projects. MR-Scout first discovers MR-encoded test cases (MTCs), and then synthesizes the encoded MRs into parameterized methods (called codified MRs), and filters out MRs that demonstrate poor quality for new test case generation. MR-Scout discovered over 11,000 MTCs from 701 OSS projects. Experimental results show that over 97% of codified MRs are of high quality for automated test case generation, demonstrating the practical applicability of MR-Scout. Furthermore, codified-MRs-based tests effectively enhance the test adequacy of programs with developer-written tests, leading to 13.52% and 9.42% increases in line coverage and mutation score, respectively. Our qualitative study shows that 55.76% to 76.92% of codified MRs are easily comprehensible for developers.

==> src/glossary.tex <==
% !TeX root = ../main.tex

{\LARGE \textbf{Glossary}}

% \textbf{Table of revision progress: }
% \begin{enumerate}
% \item Abstract and Introduction [\textbf{Ready} to revise]
%     \begin{itemize}
%       \item revised by: Prof. Cheung
%     \end{itemize}
% \item Introduction [\textbf{Ready} to revise]
% \item Formulation [\textbf{Ready} to revise]
%     \begin{itemize}
%       \item revised by: Hengcheng, Jiarong
%     \end{itemize}
% \item Methodology [\textbf{Ready} to revise]
%     \begin{itemize}
%       \item revised by: Hengcheng, Jiarong
%     \end{itemize}
% \item Evaluation [\textbf{Ready} to revise]
%     \begin{itemize}
%       \item revised by: Hengcheng 
%       \item revising by: Jiarong
%     \end{itemize}
% \item Discussion, and others [\textbf{Ready} to review]
%     \begin{itemize}
%       \item revising by: Hengcheng
%     \end{itemize}
% \end{enumerate}

\newpage
\textbf{Terminology: } 
\congying{[2023-08-17 01:00AM] terms in red needs your comments}
\begin{enumerate}
\item introduction:
    \begin{itemize}
      \item MR-encoded test case
      \item we \todo{derive} two properties
      \item \todo{validate} the relation
    \end{itemize}
\item methodology:
    \begin{itemize}
      \item Phase 1: \todo{discover} MTC based on two principal properties  /  MTC that possesses the two properties
      % \scc{please stick to one. Please make sure that consistent terminology is used in the abstract.}\congying{I choose discover}
      % \item MR \todo{deduce} \scc{deduce is better than discover}\congying{I think, we may insist on ``synthesize''? or do you think ``deduce'' is better than ``synthesize''}
      
      %\scc{(Code) Synthesis reads better than (code) deduction to me when we are talking about codified MRs. We deduce the source inputs, follow-up inputs, source outputs, and follow-up outputs from MTC.}\congying{wow, great}
      \item Phase 2: \todo{synthesize} codified MRs by ``\todo{deducing} the constituents of an encoded MR and then codifying these constituents into parameterized methods''   
      % \scc{This is why we use synthesis for the title} \congying{codify encoded MRs to parameterized methods? or codify constituents of an encoded MR to a parameterized method?}
      \item Phase 3: filter out codified MRs that demonstrate poor \todo{quality} in their applicability to new inputs for automated MT  
      %\scc{performance or quality?}\congying{quality is better}
    \end{itemize}
\item evaluation: 
    \begin{itemize}
      \item RQ1: soundness of \tool in discovering MTCs
      \item RQ2: quality of \tool codified MRs in applying to new inputs for automated MT
      \item RQ3: usefulness of \todo{codified MRs in enhancing test adequacy when integrated with automatically generated inputs}
      % \congying{what about the above sentence? In this RQ, we construct codified-MR-based test suites with \tool synthesized MRs and automatically generated inputs.}
      \item RQ4: \todo{comprehensibility} of \tool synthesized MRs for developers engaged in test maintenance and migration  
    \end{itemize}
\end{enumerate}

==> src/notes.tex <==
\section{notes for Congying}
\begin{itemize}
    \item threats to validity: time budget. "Effectiveness and Challenges in Generating Concurrent Tests for Thread-Safe Classes"
    \item threats to validity: refer to ``Modeling Readability to Improve Unit Tests'' to discuss the 
    \item in the qualitative study part, clearly discuss the existing criteria of ``good'' MR are not applicable
    \item  Prove of setGet is the target method under test.: org.ice4j.attribute.RealmAttributeTest.testSetGetRealm()
    \item ---------- (ICSE 24 submission)  
    \item what are the advantages of codified MR? In other words, what are the benefits of constructing derived MRs into Java methods? [cy: facilitate automated MR] -> ``More importantly, once the metamorphic relations are identified and implemented, the degree of automation achieved can be total if source test cases are automatically generated, e.g., randomly.''~\cite{segura2018metamorphic} to support the feasibility of auto-MT with automatically derived MRs.
    \item ``In MT, soundness is more important than completeness because: (i) every MR used in the construction of source and follow-up test cases must be genuine, other- wise, interpretation of the testing results may be meaningless; and (ii) if the user has already identified some genuine MRs, MT can still be conducted even if some actually usable candidate pairs have been incorrectly identified as unusable.'' ~\cite{chen2016metric}
    \item ``3.1 Metamorphic Relations (MRs) In this paper, without loss of generality, we assume that the targeted function (or algorithm) involves one single input and one single output. However, generalizing our results to functions with multiple inputs and outputs is straightforward.''~\cite{qiu2020theoretical} This citation may support our validation on only one source input and one follow-up input.
    \item ``More importantly, once the metamorphic relations are identified and implemented, the degree of automation achieved can be total if source test cases are automatically generated, e.g., randomly.''~\cite{segura2018metamorphic} to support the feasibility of auto-MT with automatically derived MRs.
    \item ``as clarified in a recent survey\cite{chen2018metamorphic}, some MRs require the source test cases’ outputs for generating follow- up test cases.''~\cite{sun2019metric}
    \item when describing the usage of Evosuite, we can provide a link of our tool's website, where detailed parameters for Evosuite will be provided.
    \item \textbf{MTC (metamorphic test case)} is a test case which is an instance of an MR. ``scc: In other words, the test case does not embed an MR, but an instance of the MR.'' 
    \item Relations between programs. ``Relations between programs (e.g., ``sin2(x)+cos2(x)=1'') may also help detect faults in the functions sin and cos. In future work, we will extend the definition of MRs and investigate how to infer these MRs.'' \cite{zhang2014search}
\end{itemize}

==> src/story-line.tex <==
% !TeX root = ../main.tex

{\LARGE \textbf{Story Line}}

\smalltitle{Background.} \jr{You can use this command to replace the hard-coded ones (to ease reformatting). } Metamorphic testing (MT) has been widely applied to test various programs, such as machine learning, compilers, and numerical programs. 
Metamorphic relation (MR), as the central element of MT, captures the necessary property of target systems. Effective and efficient acquisition of MRs is an important and essential task in MT~\cite{sun2019metric}. However, discovering MR is challenging, as it requires domain-specific knowledge and relies on testers' expertise. MR discovery becomes one of the most significant challenges of applying MT~\cite{2016-segura-tse} \cite{ahlgren2021testing}. 

\textbf{Limitation of existing works.} 
(1) The low degree of automation --- some MR-pattern based \cite{segura2018metamorphic}\cite{zhou2018metamorphic}, category choice based \cite{chen2016metric}\cite{sun2019metric} approaches rely on domain expertise to manually design concrete MRs. These approaches are domain-specific and unscalable.
(2) The limited application scope --- some automatic techniques are designed for specific domains (e.g., numerical programs) \cite{zhang2014search} or certain types of relations (e.g., equivalent relation, polynomial equality, and inequality relations) \cite{blasi2021memo}\cite{zhang2019automatic}.
\jr{May need more illustration to shift to our idea. How do we bypass the domain-specific limitation? Maybe you want to say that MRs in existing projects can be mined and reused in other projects? }

\textbf{Our Observation and Goal.} We find that some test cases are embedded with MR as oracles (e.g, as the test case shown in Fig.~\ref{fig:embedded-MR sample-1}, the underlying MR is ``$x=decompress(compress(x))$''). 
This motivates us to study the prevalence of MR-embedded test cases (MTC) in OSS and propose an approach, \tool, to automatically identify and extract embedded MRs from existing test cases and reuse these MRs for new test generation.% regardless of the domains/types of MRs. 
\hc{There is a gap here. We need to first explore if there are MRs encoded in the test cases and consider the extraction phase. \congying{please see if the modified version fixes this gap.}}

\textbf{Challenge.}
To date, no existing work focuses on discovering MRs from test cases. %To achieve this, we need to address two main challenges.
How to automatically identify MR-embedded test cases is challenging. 
On the one hand, MR-embedded test cases are not explicitly labeled. As the test case shown in Fig.~\ref{fig:embedded-MR sample-1}, there is no comment about the used relation. On the other hand, there is no syntactic difference between MR-embedded test cases and normal test cases. As a result, to identify test cases that possibly embed MRs, \tool needs to analyze whether there is a semantic of MR in the test cases. 

% (2) How to automatically extract and generalize embedded-MRs for new test generation is challenging.
% Actually, an MR-embedded test case is just an instance of an MR. Sometimes, a test case embeds multiple MRs \congying{Provide an example here}. To reuse the embedded MR for new test generation, \tool needs to understand the semantic \congying{May replace with ``workflow''?} of embedded MRs (such as what is the source input, and what is the follow-up input), and then replace the original source input with new source inputs.

% we need to deal with the ambiguities during the detection part. 
% extracted MR may be wrong.
% extract complete MR
% the input relation is not unavailable. -> solution/insight: use input transformation to try to build the relation between source and follow-up input.
% the input constraint problem is still existing.(future work.)
% (2) How can MRs that are embedded in MTTCs be automatically extracted and reused for test generation? 

\textbf{Solution.}
To address the above challenge, we model the semantics of MR by a set of necessary properties that are defined according to the formulation of MR and can be mechanically analyzed. \textit{The insight is that MRs actually comply with some properties which can be mechanically analyzed.}

Specifically, i) An MR is based on at least two test inputs. So, the defined property is, for an MR-embedded test case, at least two executions of the target program on these inputs are necessary. ii) An MR has a constraint over the test outputs. The defined property is, for an MR-embedded test case, at least one assertion checking the constraint over execution outputs of the target program on these inputs is necessary. %\tool determines whether a test case satisfies these properties and possibly embeds an MR.
If a test case satisfies these properties, we consider that it embeds an MR.

% To address the second challenge, the insight is that the input transformation (which transforms the source input into the follow-up input) can be leveraged to recognize the source input and follow-up input. \tool identifies the encoded input transformation to distinguish the source input and the follow-up input, and then generates new source inputs for extracted MRs to check whether an extracted MR is reusable.

% Firstly, \tool identifies the constituents of an MR in a detected MTTC. Secondly, \tool tries to generalize the embedded MRs, by codifying the embedded MRs into executable methods, and generate new inputs to extracted MR. 
% (Phase3) Test generation. The key insight is that automatic tools can be used to generate test inputs, and MRs can be reused as test oracles for new test generation. re-use embedded MRs as the oracles.

\textbf{Approach.} \tool works in three phases to identify and extract MRs for test generation. Firstly, \tool identifies MR-embedded test cases according to the defined necessary properties. 
% Secondly, \tool extracts embedded MRs by identifying the encoded input transformation to distinguish the source input and the follow-up input and codifying embedded MRs to executable methods. 
Secondly, \tool extracts embedded MRs by identifying constituents of an MR (such as the source input, the follow-up input, etc.) and codifying embedded MRs to executable methods. 
Finally, \tool employs Evosuite to generate new test inputs for extracted MRs as new test cases.


\textbf{Experiment.}
(1) RQ1, with MTCs identified by \tool, we study the prevalence, constituents, and tested programs' domains of MTCs in open-source projects.
(2) RQ2, we evaluate the soundness of \tool in identifying and extracting MRs, by manually analyzing the identified MTCs and codified MRs. We release the dataset of identified MTCs and codified MRs. 
(3) RQ3, we evaluate the usefulness of codified MR for test generation, and analyze if there is fault detection capability improvement (i.e., the improvement of line coverage and mutation score) \scc{what is fault capability improvement? improved coverage?}  by codified-MR-based test cases, on top of original human-written test cases and Evosuite-generated test cases. \scc{pay attention to the consistency of tense.}
We take original human-written test suites and Evosuite-generated test suites as baselines.
\scc{baselines?}
% \congying{we take original human-written test suites and Evosuite-generated test suites as baselines.}

\textbf{Contributions.}
(1) We propose \tool, the first approach that automatically identifies and extracts MRs from existing test cases.
(2) [RQ1] We study the status quo of MTC in open-source projects, in terms of the prevalence, constituents, and tested programs' domains.
(3) [RQ2] We release the dataset of manually evaluated MTCs and codified MRs.  
(4) [RQ3] We conduct extensive experiments to demonstrate the soundness of \tool and the usefulness of codified MRs for test generation. 

==> table/expertise.tex <==
\begin{tabular}{l|rrr}
\toprule
\multirow{2}{*}{\textbf{Experience and Skills}} & 
\multicolumn{3}{c}{\textbf{ Participants }} \\
\cmidrule(l{1pt}r{1pt}){2-4} 
      & \textbf{A} & \textbf{B} & \textbf{C} \\
\midrule
Years of programming in Java                    & 3          &   5    &  7  \\
Years of using Junit framework                  & 3          &   4    &  7 \\
Years of researching on MT-related topics       & 2          &   1    &  1 \\
\bottomrule
\end{tabular}

% Participants

==> table/prevalence.tex <==
\begin{tabular}{rrr}
\toprule
\textbf{\# Collected Projects}   & \textbf{\# Projects w/ MTC} & \textbf{Percentage} \\
\midrule
4,068        & 701          & 17.23\%               \\
% \bottomrule
% \toprule
\midrule
\textbf{\# Collected Test Cases} & \textbf{\# Identified MTCs}       & \textbf{Percentage}                  \\
\midrule
1,021,129    & 11,350       & 1.11\%                 \\
\bottomrule
\end{tabular}

==> table/rq-usefulness-originalTestCase.tex <==
\begin{tabular}{|c|ccc|}
\hline
\multirow{2}{*}{\textbf{Metrics}} & \multicolumn{3}{c|}{\textbf{VS. OTC}}                                                       \\ \cline{2-4} 
                                  & \multicolumn{1}{c|}{\textbf{OTC}} & \multicolumn{1}{c|}{\textbf{OTC+CMR}} & \textbf{Impro.} \\ \hline
Line Coverage                     & \multicolumn{1}{c|}{0.3791}       & \multicolumn{1}{c|}{0.5032}           & +32.72\%        \\ \hline
Test Strength                     & \multicolumn{1}{c|}{0.5519}       & \multicolumn{1}{c|}{0.6579}           & +19.19\%        \\ \hline
P. of Covered   Mutants           & \multicolumn{1}{c|}{0.3565}       & \multicolumn{1}{c|}{0.4813}           & +34.98\%        \\ \hline
Mutation Score                    & \multicolumn{1}{c|}{0.2458}       & \multicolumn{1}{c|}{0.3581}           & +45.7\%         \\ \hline
\end{tabular}

==> table/rq_soundness_manual_investigation.tex <==

\begin{tabular}{|l|l|l|l|}
\hline
\# \textbf{Samples}                & \textbf{TP}             & \textbf{FP}            & \textbf{Unclear}     \\ \hline
\multicolumn{1}{|r|}{100} & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{3} & \multicolumn{1}{r|}{2} \\ \hline
\end{tabular}

==> table/topN_pojs_with_MTCs.tex <==
\begin{center}
\renewcommand{\arraystretch}{1.2}
\begin{tabularx}{\linewidth}{p{2.9cm}Xrr}
% \begin{tabularx}{\linewidth}{p{2.9cm}p{6.5cm}rr} 
\toprule
\textbf{Projects}
& \textbf{Description}
& {\textbf{\#. MTCs}}
& {\textbf{\%. MTCs}}
\\ 
\midrule
eclipse-collections      & Java collections framework                                                                            & 683    & 6.20\%   \\ 
jfreechart               & Charting and data visualization library                                                               & 321    & 13.70\%  \\ 
spring-analysis-note     & Framework for dependency injection, data access, transaction management, web   development, and more. & 310    & 1.80\%   \\ 
gridgain                 & Data fabric and distributed computing platform                                                        & 290    & 1.90\%   \\ 
OpenOLAT                 & Web-based e-learning platform                                                                         & 274    & 5.50\%   \\ 
ignite                   & Distributed database for high-performance computing                                                   & 264    & 1.70\%   \\ 
flexmark-java            & Library for parsing CommonMark compliant markdown                                                     & 197    & 15.00\%  \\ 
JMRI                     & Model railroad digital command and control software                                                   & 196    & 1.30\%   \\ 
itext7                   & PDF creation and manipulation library                                                                 & 187    & 2.30\%   \\ 
rskj                     & RSK blockchain and smart contract platform                                                            & 186    & 4.00\%   \\ 
dhis2-core               & Information system for data capture, management, validation, analytics and   visualization            & 183    & 3.00\%   \\ 
trino                    & Distributed SQL query engine for big data analytics                                                   & 173    & 1.60\%   \\ 
activemq-artemis         & Asynchronous messaging system                                                                         & 167    & 2.20\%   \\ 
datasketches-java        & Library of stochastic streaming algorithms                                                            & 147    & 7.70\%   \\ 
hetu-core                & Engine for in-situ data analytics                                                                     & 139    & 1.90\%   \\ 
coherence                & Platform for building grid-based applications and storing data.                                       & 126    & 2.00\%   \\ 
swim                     & Platform for building stateful microservices, streaming APIs, and real-time UIs                       & 124    & 7.30\%   \\ 
cantaloupe               & Dynamic image server                                                                                  & 119    & 3.50\%   \\ 
hedera-services          & Ledger for cryptocurrency and smart contracts                                                         & 115    & 2.20\%   \\ 
androidx                 & Suite of libraries, tools, and guidance to help develop apps                                          & 111    & 1.00\%   \\ 
dsl-json                 & Java JSON library designed for performance                                                            & 107    & 16.70\%  \\ 
morpheus-core            & Distributed publish-subscribe messaging platform                                                      & 104    & 19.20\%  \\ 
pulsar                   & Distributed publish-subscribe messaging platform                                                      & 100    & 1.70\%   \\ 
mapbox-gl-native-android & Library for interative vector maps                                                                    & 97     & 8.90\%   \\ 
flow                     & Platform for building websites                                                                        & 97     & 1.70\%   \\ 
\bottomrule
\end{tabularx}
\end{center}
